Cybersickness-aware Tile-based Adaptive 360{\deg} Video Streaming

In contrast to traditional videos, the imaging in virtual reality (VR) is 360{\deg}, and it consumes larger bandwidth to transmit video contents. To reduce bandwidth consumption, tile-based streaming has been proposed to deliver the focused part of the video, instead of the whole one. On the other hand, the techniques to alleviate cybersickness, which is akin to motion sickness and happens when using digital displays, have not been jointly explored with the tile selection in VR. In this paper, we investigate Tile Selection with Cybersickness Control (TSCC) in an adaptive 360{\deg} video streaming system with cybersickness alleviation. We propose an m-competitive online algorithm with Cybersickness Indicator (CI) and Video Loss Indicator (VLI) to evaluate instant cybersickness and the total loss of video quality. Moreover, the algorithm exploits Sickness Migration Indicator (SMI) to evaluate the cybersickness accumulated over time and the increase of optical flow to improve the tile quality assignment. Simulations with a real network dataset show that our algorithm outperforms the baselines regarding video quality and cybersickness accumulation.

==> 7-Implementation.tex <==
\section{Implementation}

To evaluate the performance of our system, we have implemented a prototype that includes a 360-degree video player developed in Unity, a local server handling the requested for the videos. The architecture of our system is described as follows: we use ERP format 360 videos, it was cropped and clipped in the server. After the video tiles are ready, our algorithm dynamically allocates the quality levels of each tile and also decides the size of the viewport and whether to activate DoF simulation based on the prediction of user head movements \cite{furion,360vid-ProbDASH} and the cost function. the video content will be transmitted to the client through ALVR \cite{ALVR}, a software that works as a VR rendering engine and also a UDP-based streaming system.

\subsection{Hardware}
A PC with Intel i7-9700 CPU, Nvidia 2070 super GPU, 24 GB RAM as our server. It connects to an Asus AC68u AP using an Ethernet cable. We use Oculus Quest VR headset as our client that connects to the AP through 5Ghz WiFi. The VR headset communicates with the server via an AP that can achieve 440Mbps TCP throughput for one device.

\subsection{Video Setup}
First, we encode video contents by FFmpeg\cite{FFMPEG} into five bitrate levels with CRF 43, 38, 33, 28, and 23 \cite{360vid-Flare}. In order to get the desired number of video tiles, we then cropped the video into 6x8 tiles with FFmpeg filters. Finally, we separate our video tiles into one-second segments \cite{360vid-ProbDASH,360vid-EPASS360} and store them in the server.

\subsection{Server Component}
As shown in Fig. \ref{fig:system}, 360 videos will be processed and stored inside the server. Our server contains several key components as follow: 
\begin{enumerate}
    \item Encoder: This component encodes video sources to various bitrate levels with H.264 of libx264 library.
    \item Cropper: This module spatially cut the video frame into a specific number of video tiles.
    \item Clipper: Clipper splits video tiles into segments of short duration to accelerate the changing process of tile quality levels. Noted that the encoder, cropper, and clipper can be integrated into one component by modifying the encoder, but it is rather complicated to implement.
    \item Rate adaption: The rate adaption component dynamically adjusts the quality level of tiles, the viewport size, and the DoF simulation based on our algorithm and the result of viewport prediction to satisfy the request of the user.
    \item Video Player: We attached the processed video tiles to a video player in the Unity \cite{Unity} system, then stream the whole frame to the user with ALVR \cite{NTUedge}.
\end{enumerate}

\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth] {Fig/system.png}
\caption{System Architecture}
\label{fig:system}
\end{figure}

\subsection{Client Component}
The client component in our system is implemented based on the open-source project ALVR which is written in JAVA. In order to show the characteristics of our system, we add extra functions to the client. First, a user's orientation is collected by the sensor on the VR headset. Next, we can revise the position of the viewport based on the head rotation of the user on the Pitch and Yaw axes. Besides adjusting the viewport size of the client, we have built an orientation prediction model \cite{360vid-ProbDASH}, which is a linear regression model trained offline on the server and updated to the client periodically. Then the client can fetch the video tiles according to the viewport prediction results. After receiving the packets sent from the server, the client decodes it locally and adjusts the frame distortion to ready the video for display.
\par
% \emph{Why ALVR?}
% The reason we choose ALVR as our streaming agent instead of other choices is that our system is built upon Unity, which allows our work to support both 360\textdegree video playback and VR games. Also, it is important for users to have an untethered experience, so we use a standalone VR headset as our client. In this case, ALVR has adequate support on streaming content from the server to clients.

\subsection{User Study}

We applied a three-session mixed experimental design, testing the effectiveness of ETSCAA against two baselines, a 360\textdegree video streaming algorithm \cite{360vid-EPASS360} and an optimized cybersickness alleviating function \cite{Sickness-FoV-2}. The average bitrate setting and bandwidth traces follow the dataset in \cite{360vid-EPASS360}. A total of 40 participants took part, with an age range of 20 to 28 years old. 5 participants were female, and the rest were male. In the two sessions, the participants first complete the pre-exposure Simulator Sickness Questionnaire (SSQ) \cite{SSQ}. SSQ consists of 16 questions. Each question asks the participants to rate the severity of a symptom that is related to cybersickness. The final score is then calculated by the weighted average of the 16 symptom ratings. Next, they are asked to watch a 4K 360\textdegree roller coaster video \cite{360vid-EPASS360} for 10 minutes. The system dynamically controls the bitrate level of each tile and the cybersickness alleviating functions based on the algorithms (one session with ETSCAA and one with EPASS360) during the playback of the video. Finally, the participants complete the post-exposure SSQ. They also need to fill a video quality questionnaire that includes multiple questions. Noted that half of the participants experience the ETSCAA session first and the others experience the EPASS360 session first to balance the effect of testing order. Each participant rests for 30 minutes between the two sessions to reset the cybersickness level \cite{Sickness-TempAspect}.
